Extremes of the 2d scale-inhomogeneous discrete Gaussian free field: Sub-leading order and exponential tails

This is the first of a three paper series in which we present a comprehensive study of the extreme value theory of the scale-inhomogeneous discrete Gaussian free field. This model was introduced by Arguin and Ouimet who computed the first order of the maximum. In this first paper we establish tail estimates for the maximum value, which allow to deduce the log-correction to the order of the maximum and tightness of the centred maximum. Our proofs are based on the second moment method and Gaussian comparison techniques.

==> abstract.tex <==
This is the first of a three paper series in which we present a comprehensive study of the extreme value theory of the scale-inhomogeneous discrete Gaussian free field. This model was introduced in \cite{MR3541850} by Arguin and Ouimet in which they computed the first order of the maximum. In this first paper we establish the log-correction to the order of the maximum and establish tightness of the centred maximum. Our proofs are based on the second moment method and Gaussian comparison techniques.

==> acknowledgement.tex <==
I want to thank my advisor Prof. Dr. Anton Bovier for his support, advice, discussions and, of course, introducing me into this research area and thus, drawing my interest to it. I would also like to thank Dr. Lisa Hartung and Dr. Sebastian Andres for inspirations, advice and the opportunity to deepen my knowledge on this and related subject matters.
Last but not least, I want to thank my parents for their enduring support.

==> auxiliary_processes.tex <==
The key idea of the proofs of \autoref{theorem:thm_second_order_correction} and \autoref{theorem:thm_tightness} is as in the case of the DGFF \cite{MR2846636}. We construct Gaussian fields with index set $V_N$ that approximate the correlation structure of the scale-inhomogeneous Gaussian free field and then make multiple use of Gaussian comparison, namely the Sudakov-Fernique inequality and Slepian's Lemma (see \autoref{thm:sudakov} and \autoref{thm:slepian}). This permits us to analyse the auxiliary processes instead of the original field, which is simpler as they possess something close to a hierarchical structure. The approximation of the correlation structure can be reduced to approximating the Euclidean distance. In this section we introduce in analogy to \cite{MR2846636} the needed auxiliary processes and estimate their correlations. 


==> def_gff.tex <==
We first want to introduce the Gaussian Free Field (GFF) and investigate some of its key properties.
Let $N \in \mathbbm{N}$, $V_N \coloneqq ([0,N]\cap \mathbbm{Z})^2$ of side length $N+1$.


For $B \subseteq V_N$ we write $\mathcal{F}_B \coloneqq \sigma()

==> ldp.tex <==
In order to prove our theorem, we prove an upper and a lower bound. Therefore, we need to identify paths along which we can find particles reaching a certain level of height, at all different scales, of course with a positive probability.
For $0<\gamma<\gamma^*$, we call $v\in V_N$ a $\gamma-$high point, if $\psi_v \geq \gamma \log(N^2)$. We aim to identify a path $\lambda \rightarrow L_N^{\gamma}(\lambda)$ above which we can find at least one $\gamma-$high point throughout all scales. We write $L_N^*$ for the corresponding optimal path in the case of the maximum level $\gamma^*$. These paths are crucial to prove tight upper and lower bounds in the subsequent proofs.
\\ The following first moment, large deviation argument, taken from \cite{MR3541850}, is quite general and common, as it allows for more general increments as well as tree structures. The presentation here should be a heuristic instruction how to obtain such paths:
It is somewhat intuitive to consider the necessary gains $\nabla \gamma_i$  in height between two subsequent scales in order to reach a given height. The height levels $\gamma_i$ at scales $\lambda_i$ are unknown variables for us for the time being.
We consider the points $v \in V_N$ that reach these levels, so we define:
\begin{equation}
	\Lambda_{N,M} \coloneqq \{ v \in V_N\,:\,\nabla \psi_v(\lambda_i)\geq \nabla \gamma_i \log(N^2),\, \text{for all}\, i \in \{1,\dotsc,M\} \},
\end{equation}
with  $\gamma_0 \coloneqq 0.$ Per definition, points $v \in \Lambda_{N,M}$ certainly reach at least height $\gamma_M \log(N^2)$ and thus $|\Lambda_{N,M}|< \left|\left\{ v\in V_N \,:\, \psi_v \geq \gamma_M \log(N^2) \right\}\right|.$ In words, $\left|\Lambda_{N,M}\right|$ is a lower bound on the number of particles in $V_N$ reaching at least level $\gamma_M \log(N^2)$. In addition, we want to consider points that have certain gains of height at least up to an intermediate scaling $\lambda_k$. Because of correlations, we can restrict ourselves to consider only representatives in $R_{\lambda_k}$:
\begin{equation}
	\Lambda_{N,k} \coloneqq \left\{ v \in R_{\lambda_k} \,:\, \nabla\psi_v(\lambda_i)\geq \nabla \gamma_i \log(N^2), \, \text{for all} \, i \in \{1,\dotsc,k \} \right\}.
\end{equation}
 Since the number of representatives in $R_{\lambda_k}$ is $N^{2\lambda_k}$, we have using independent increments:
\begin{equation}
	\mathbbm{E} [|\Lambda_{N,k}|]= N^{2\lambda_k}\prod_{i=1}^{k} \mathbbm{P}\left(\nabla \psi_v(\lambda_i)\geq 2 \nabla \gamma_i \log(N)\right).
\end{equation}
On the probability terms, we want to apply the standard Gaussian estimate due to Gordon (see \cite{gordon1941}), which states that for a normal random variable $X \sim N(0,\sigma^2)$ and $z \in \mathbbm{R}_+$, it holds
\begin{equation}\label{gaussian_estimate}
	\left(1-\frac{\sigma^2}{z^2}\right)\frac{\sigma}{\sqrt{2\pi}z} \exp\left(-\frac{z^2}{2\sigma^2}\right)\leq \mathbbm{P}(X\geq z)\leq \frac{\sigma}{\sqrt{2\pi}z}\exp\left(- \frac{z^2}{2\sigma^2}\right).
\end{equation}
Because the contribution of the boundary to the variance of particles is negligible in the limit, we now assume $\mathrm{Var}(\nabla \psi_v (\lambda_i))= \sigma_i^2 \nabla \lambda_i \log(N) + O(1).$ Moreover, we have by definition and the tower-property of conditional expectation:
\begin{align}
	\mathbbm{E}[\nabla \psi_v (\lambda_i)]&= \mathbbm{E}[\sigma_i \nabla \phi_v(\lambda_i)-\sigma_{i-1}\nabla \phi_v(\lambda_{i-1})]\nonumber\\&= \mathbbm{E}[\sigma_i (\mathbbm{E}[\phi_v|\mathcal{F}_{\partial{[v]_{\lambda_i}} \cap [v]_{\lambda_i}^c }] - \mathbbm{E}[\phi_v|\mathcal{F}_{\partial{[v]_{\lambda_{i-1}}} \cap [v]_{\lambda_{i-1}}^c }])\nonumber \\&\quad-\sigma_{i-1}( \mathbbm{E}[\phi_v|\mathcal{F}_{\partial{[v]_{\lambda_{i-1}}} \cap [v]_{\lambda_{i-1}}^c }] - \mathbbm{E}[\phi_v|\mathcal{F}_{\partial{[v]_{\lambda_{i-2}}} \cap [v]_{\lambda_{i-2}}^c }]) ]\nonumber \\&= \mathbbm{E}[\sigma_i(\phi_v-\phi_v)-\sigma_{i-1}(\phi_v-\phi_v)]=0.
\end{align}
Thus, we have $\nabla \psi_v(\lambda_i) \sim N(0,\sigma_i^2 \nabla \lambda_i \log(N) + O(1))$ and can therefore apply the estimate \eqref{gaussian_estimate} to obtain:
\begin{equation}\label{est1}
	c \frac{N^{2\lambda_k}}{\sqrt{\log(N)^k}} N^{-2\sum_{i=1}^{k}\frac{(\nabla \gamma_i)^2}{\sigma_i^2 \nabla \lambda_i}} \leq \mathbbm{E} \left[\left|\Lambda_{N,k}\right|\right] \leq C \frac{N^{2\lambda_k}}{\sqrt{\log(N)^k}} N^{-2\sum_{i=1}^{k}\frac{(\nabla \gamma_i)^2}{\sigma_i^2 \nabla \lambda_i}},
\end{equation}
where $c,C>0$ are some finite constants.
Rewriting \eqref{est1} yields:
\begin{equation}\label{est2}
	\lim_{N \rightarrow \infty} \frac{\log\left(\mathbbm{E}[|\Lambda_{N,k}|]\right)}{2 \log(N)}= \sum_{i=1}^{k}\left(\nabla \lambda_i - \frac{(\nabla \gamma_i)^2}{\sigma_i^2 \nabla \lambda_i}\right).
\end{equation}
We expect that at each scale $\lambda_k \text{ , }k\in \{1,\dotsc,M\}$, it exists a representative in $R_{\lambda_k}$ reaching the prescribed height $\gamma_M$ at level $\lambda_M$. Taking into account this constraint, considering \eqref{est2}, we expect to find the first order of the maximum level by maximizing the following quantity:
\begin{align}\label{equation:kkt_constraints}
	&\gamma_M =\sum_{i=1}^{M} \nabla \gamma_i &\text{under the constraints } &\sum_{i=1}^{k}\left(\nabla \lambda_i - \frac{(\nabla \gamma_i)^2}{\sigma_i^2 \nabla \lambda_i}\right) \geq 0, \, 1\leq k\leq M.
\end{align}
This optimization problem can be solved by applying the Karush-Kuhn-Tucker (KKT) Theorem:
\begin{thm}[Karush-Kuhn-Tucker Theorem, cp.{\cite[Theorem 6.1]{MR1402910}}]
	Let $n,M\in \mathbbm{N}$ be two non-zero integers and $D\subset \mathbbm{R}^n$ be an open set. Let $f:D\rightarrow D$ be the function to optimize and $g_k:D\rightarrow \mathbbm{R}$, $1\leq k \leq M$, the constraint functions, so that $U\coloneqq \{x\in D:\,g_k(x)\geq 0\, \forall k \in\{1,\dotsc,M\}\}$ is the constrained set.
	Suppose that 
	\begin{enumerate}
		\item $f$ restricted to $U$ has a local maximum at $x^* \in U$,
		\item $f$ is Fréchet differentiable at $x^*$,
		\item $\{g_k\}_{1\leq k \leq M}$ are Fréchet differentiable at  $x^*$.
	\end{enumerate}
	If these conditions hold, then there exists a vector $(\mu_1,\dotsc,\mu_M)\in \mathbbm{R}^M$, such that the following holds for any $k\in \{1,\dotsc,M\}:$
	\begin{enumerate}
		\item $\nabla f(x^*)+\sum_{k=1}^{m}\mu_k g_k(x^*)=0$,
		\item $g_k(x^*)\geq 0$,
		\item $\mu_k\geq 0$,
		\item $\mu_k g_k(x^*)=0$.
	\end{enumerate}
\end{thm}
Regarding Equation \eqref{equation:kkt_constraints}, we take as objective function $f=\sum_{i=1}^{M}x_i$ and as constraint functions $g_k(x)=\sum_{i=1}^{k}\left(\nabla \lambda_i - \frac{x_i^2}{\sigma_i^2 \nabla \lambda_i}\right)$. We denote the unique solution by $\gamma_i^*=\mathcal{I}_{\sfrac{\sigma^2}{\bar{\sigma}}}(\lambda_{i-1},\lambda_i),$ for $i=1,\dotsc,M$. The polygonal line linking the points $(0,0),(\lambda_1,\gamma_1^*),\dotsc,(\lambda_M,\gamma_M^*)$ is given by
\begin{equation} \label{opt_path_max}
	\frac{1}{2\log N}L_N^*(s) =\int_{0}^{s} \frac{\sigma^2(r)}{\bar{\sigma}(r)}\mathrm{d}r = \mathcal{I}_{\sfrac{\sigma2}{\bar{\sigma}}}(s), \, \text{for} \, s \in [0,1].
\end{equation}
This is called the "optimal path for the maximum." Note that the optimal path coincides with its concave hull at the points $\lambda^l$, exactly where $\bar{\sigma}$ jumps, that is
\begin{equation}
	L_N^*(\lambda^l) \coloneqq \hat{L}_N^*(\lambda^l)=2\log(N) \hat{\mathcal{I}}_{\sfrac{\sigma^2}{\bar{\sigma}}}(\lambda^l)=2\log(N)\mathcal{I}_{\bar{\sigma}}(\lambda^l), \quad 1 \leq l \leq m.
\end{equation}
Now, we try to find "optimal paths" for $\gamma-$high points for general $\gamma$ with $0<\gamma<\gamma^*$. For this purpose we set $\gamma_M=\gamma$ and derive analogously to Equation \eqref{est2}
\begin{equation}\label{opt2}
	\lim_{N\rightarrow \infty} \frac{\log(\mathbbm{E}[|\Lambda_{N,M}|])}{2\log(N)}= \sum_{i=1}^{M-1} \left(\nabla \lambda_i- \frac{(\nabla \gamma_i)^2}{\sigma_i^2 \nabla \lambda_i}\right)+\left(\nabla \lambda_M - \frac{(\gamma - \gamma_{M-1})^2}{\sigma_M^2 \nabla \lambda_M}\right).
\end{equation}
Then just as in the case for the maximum we maximize the quantity on the right-hand side of \eqref{opt2} with respect to $\gamma_1, \dotsc, \gamma_{M-1}.$ under the constraint that we can find at least one representative at each scale, namely
\begin{equation}
	\sum_{i=1}^{k}\left(\nabla \lambda_i - \frac{(\gamma_i)^2}{\sigma_i^2 \nabla \lambda_i}\right)\geq 0, \quad 1\leq k\leq M-1.
\end{equation}
Applying Karush-Kuhn-Tucker once again, we obtain the "optimal path" for $\gamma-$high points, assuming $\gamma^{l-1}<\gamma<\gamma^l$:
\begin{equation} \label{opt_path}
	L_N^{\gamma}(s) \coloneqq \begin{cases}
		L_N^*(s) &, \text{ } 0\leq s \leq \lambda^{l-1} \\
		L_N^*(\lambda^{l-1})+ 2\gamma \log(N) \frac{\mathcal{I}_{\sigma^2}(\lambda^{l-1},s)}{\mathcal{I}_{\sigma^2}(\lambda^{l-1},1)} - L_N^*(\lambda^{l-1})   &, \text{ }\lambda^{l-1}\leq s \leq 1.
	\end{cases}
\end{equation}
Observe that on the interval $[0, \lambda^{l-1}]$, this paths coincides 
with the optimal path for the maximum (cf. Equation \eqref{opt_path_max}). Moreover, $L_N^{\gamma}$ is continuous and converges uniformly to $L_N^*$ as $\gamma \rightarrow \gamma^*$.

==> lower_bound.tex <==
In this section our goal is to prove a corresponding lower bound on the expected maximum of the scale-inhomogeneous DGFF. In a first step, we  prove that the expected maximum of $\psi_N$ can be bounded from below by a truncated version of the MIBRW $S_N$. This is done by applying Slepian's lemma. The truncation of the first few largest scales gives us additional independence which we want to exploit to obtain a summable lower bound. In a second step, we prove a suitable lower bound on the MIBRW via a second moment computation on the number of particles reaching the desired level of height. Recall the definition of the MIBRW in \eqref{equation:def_MIBRW}.
\begin{definition}[Truncated MIBRW]
	Let $0 \leq k_0 \leq n$ be an integer. We define the truncated modified inhomogeneous branching random walk (TMIBRW) by
	\begin{equation}
		S_z^{N,k_0} = \sum_{k=k_0}^{n} \sum_{B \in \mathcal{B}_k(z)} 2^{-k} \sigma\left(\frac{n-k}{n}\right) b_{k,B}^N,
	\end{equation}
	and set $S_{N,k_0}^* \coloneqq \max_{v \in V_N} S_z^{N,k_0}.$
\end{definition}
For $v,w \in V_N$, let $\varrho_{N,k_0}(v,w)= \mathbbm{E}\left[(S_v^{N,k_0}-S_w^{N,k_0})^2 \right]$. We collect some basic properties of $\varrho_{N,k_0}$.
\begin{lemma} \label{lemma:truncated_var_lemma}
	The function $\varrho_{N,k_0}$ satisfies:
	\begin{itemize}
		\item[i.] $ \varrho_{N,k_0}(v,w) \text{ decreases in } k_0. $
		\item[ii.] $ \limsup\limits_{k_0 \rightarrow \infty} \limsup\limits_{N \rightarrow \infty} \sup\limits_{v,w\in V_N: \, d_N(v,w)\leq 2^{\sqrt{k_0}} } \varrho_{N,k_0}(v,w) = 0. $
		\item[iii.] $\text{There is a function }g: \mathbbm{Z}_+ \rightarrow \mathbbm{R}_+ \text{ such that } g(k_0) \rightarrow \infty$ $\text{ as } k_0 \rightarrow \infty,
		  \text{and for } v,w \in V_N \text{ with }\nonumber \\ d^N(v,w)\geq 2^{\sqrt{k_0}}$ and $2^n> k_0$, we have
		  \begin{align}
		  	\varrho_{N,k_0} (v,w) \leq \varrho_{N,0}(v,w) - g(k_0).
		  \end{align}
	\end{itemize}
	\begin{proof} 
		For $v=(v_1,v_2)\neq w=(w_1,w_2) \in V_N$ and $i=1,2$, let $r_i(v,w)= \min(|v_i-w_i|,|v_i-w_i-N|,|v_i-w_i+N|)$. Note that in the definition of the MIBRW the number of common boxes of side length $2^k$ for $v,w\in V_N$ is given by $[2^k-r_1(v,w)][2^k-r_2(v,w)]$. And so we may compute the order of fluctuations by counting the number of unshared boxes, i.e.\allowdisplaybreaks
		\begin{align} 
			\varrho_{N,k_0}(v,w)&= \mathbbm{E}\left[(S_v^{N,k_0}- S_w^{N,k_0})^2\right]= 2 \mathbbm{E}\left[(S_v^{N,k_0})^2] -2 \mathbbm{E}[S_v^{N,k_0}S_w^{N,k_0}\right]\nonumber\\
			&=2 \sum_{k=k_0}^{n} 2^{-2k} 2^k 2^k \sigma^2\left(\frac{n-k}{n}\right)  \nonumber\\ 
			 &\qquad+2\sum_{k=\ceil*{\log_2(d_\infty^N(v,w)+1)}\vee k_0}^{n} 2^{-2k} \sigma^2\left(\frac{n-k}{n}\right) \left(-2^k+ r_1(v,w)\right)\left(-2^k + r_2(v,w)\right) \nonumber \\ 
			 &=2\sum_{k=k_0}^{\ceil*{\log_2(d_\infty^N(v,w)+1)}\vee k_0} \sigma^2\left(\frac{n-k}{n}\right)\nonumber\\
			 &\qquad+2 \sum_{k=\ceil*{\log_2(d_\infty^N(v,w)+1)}\vee k_0}^{n} \sigma^2\left(\frac{n-k}{n}\right) \left(\frac{r_1(v,w)}{2^k}+\frac{r_2(v,w)}{2^k}- \frac{r_1(v,w)r_2(v,w)}{4^k}\right).
		\end{align}
		From this representation the first two properties are immediate. For the third statement, note that for $\log_2(d_\infty^N(v,w)) \geq \sqrt{k_0} -1$,
		\begin{equation}
			\varrho_{N,0}(v,w) - \varrho_{N,k_0}(v,w) \geq \sqrt{k_0} \min_{0\leq k \leq \sqrt{k_0}}\sigma^2\left(\frac{n-k}{n}\right)-1.
		\end{equation}
	\end{proof}
\end{lemma}
In addition, we need a comparison between the maxima of the $(\sigma,\lambda)-$DGFF and the truncated MIBRW.
\begin{cor}\label{cor:corollary_2}
	There is a constant $k_0>0,$ such that for all $N=2^n$ large enough and all $v,w \in V_N$,
	\begin{equation}
		\mathbbm{E}\left[\psi_N^*\right] \geq \sqrt{\log(2)} \mathbbm{E}\left[S_{\sfrac{N}{4},k_0}^*\right].
	\end{equation}
	\begin{proof}
		We have
		\begin{equation}
			\psi_N^* \geq \max_{v \in V_{\sfrac{N}{4}}+(\sfrac{N}{2},\sfrac{N}{2})} \psi_v^N.
		\end{equation}
		On the other hand, for $v,w \in V_{\sfrac{N}{4}}$ we get with statement $iv.$ in \autoref{lemma:cov_comp}
		\begin{equation} \label{cor2_equ1}
			\mathbbm{E}\left[(\psi_{x+(\sfrac{N}{2},\sfrac{N}{2})}^N- \psi_{y+(\sfrac{N}{2},\sfrac{N}{2})}^N)^2\right] \geq \log(2)\mathbbm{E}\left[(S_x^{\sfrac{N}{4}}- S_y^{\sfrac{N}{4}})^2\right] -C.
		\end{equation}
		Applying \autoref{lemma:truncated_var_lemma} and Sudakov-Fernique to \eqref{cor2_equ1}, we obtain
		\begin{equation}
			\mathbbm{E}\left[\psi_N^*\right] \geq \mathbbm{E}\left[\max_{v \in V_{\sfrac{N}{4}+(\sfrac{N}{2},\sfrac{N}{2})}} \psi_v^N\right] \geq \sqrt{\log(2)} \mathbbm{E}\left[ S_{\sfrac{N}{4},k_0}^*\right],
		\end{equation}
		where we compensated the constant $C>0$ in \eqref{cor2_equ1} by a cut-off of the first $k_0$ contributions of $\{S^{\sfrac{N}{4}}_v \}_{v \in V_{N^{'}} }.$
	\end{proof}
\end{cor}

==> lower_bound_mibrw.tex <==

	Now, we can turn to prove a corresponding upper bound on the $2$nd moment of $h_N$.
	\begin{proof}[Proof of \autoref{lemma:upboundon2ndmoment}:]
		As in the previous proof, we start with the case of one effective parameter, i.e. $m=1$ and may again assume $\mathcal{I}_{\sigma^2}(s)<\hat{\mathcal{I}}_{\sigma^2}(s)$ for $s\in (0,1)$.
		For $v,w \in V_N$, let $r(v,w)=n-\lceil\log_2(d_N^\infty(v,w)+1)\rceil$ denote the number of independent increments in the processes $S_v^N(k)$ and $S_w^N(k^{'})$. Using this we may rewrite the second moment, i.e.
		\begin{align}
			\mathbbm{E}\left[h_N^2\right]=\sum_{v,w\in V_N{\prime}} \mathbbm{P}\left(C_v^N(t^1)\cap C_w^N(t^1)\right)= \sum_{k=0}^{n}\sum_{\substack{v,w \in V_N^{'}\\r(v,w)=k}} \mathbbm{P}\left(C_v^N(t^1)\cap C_w^N(t^1)\right).
		\end{align}
		The right hand side may be bounded from above by
		\begin{align}
			\mathbbm{E}[h_N]^2+\mathbbm{E}[h_N] + \sum_{k=1}^{n-1} \sum_{\substack{v,w \in V_N^{'}\\r(v,w)=k}} \mathbbm{P}\left(C_v^N(t^1)\cap C_w^N(t^1)\right). \label{equation:1pcase_2nd_moment_1}
		\end{align}
		We need to bound the double sum in \eqref{equation:1pcase_2nd_moment_1} which we do by bounding each summand. Fix $v,w \in V_N^{'}$ with $r(v,w)=r=k \in \{1,\dotsc,n-1\}$. We set $B_{k,n}(x)\coloneqq x-s_{k,n}(x)[-f_{r,n},f_{r,n}]$. Dropping the constraint for $w$ up to time $r$, we have
		\begin{align}
			\mathbbm{P}\left(C_v^N (t^1)\cap C_w^N(t^1) \right)\leq &\mathbbm{P}\left(C_v^N(t^m) \cap C_w^N(r)\right)\max_{x\in I_n(1)} \mathbbm{P}\left(S_w^N(t^1)-S_w^N(r)\in B_{r,n}(x)\right)\nonumber\\ \leq &\mathbbm{P}\left(C_v^N(t^m)\right) \max_{x \in I_n(1)}\mathbbm{P}\left(S_w^N(t^1)-S_w^N(r)\in B_{r,n}(x)\right).
		\end{align}
		For fixed $v \in V_N^{'}$, the number of points $w\in V_N^{'}$ satisfying $d_N^{\infty}(v,w)\in [2^k,2^{k+1}],$ i.e. when $r(v,w) \in [n-k-1,n-k]$, is bounded by $c_1 2^{2k}=2^{2(t^1-r)}$ for a $c_1>0$. Therefore, we can bound the last summand in \eqref{equation:1pcase_2nd_moment_1} from above by
		\begin{align}\label{equation:max_P_1}
			c_1\mathbbm{E}[h_N]  \sum_{r=1}^{n-1}2^{2(t^1-r)}\max_{x \in I_n(1)}\mathbbm{P}\left(S_v^N(t^1)-S_v^N(r)\in B_{r,n}(x)\right). 
		\end{align}
		Next, we set $A_{r,n,x}\coloneqq\mathbbm{P}\left(S_v^N(t^1)-S_v^N(r)\in B_{r,n}(x)\right)$ and bound this for any $x\in I_n(1)$, i.e.
		\begin{align}
			\mathbbm{P}\left(S_v^N(t^1)-S_v^N(r)\in B_{r,n}(x)\right) &=\frac{1}{\sqrt{2 \pi \mathcal{I}_{\sigma^2} (\sfrac{r}{n},\lambda^1)n}}\int_{x-s_{r,n}(x)-f_{r,n}}^{x-s_{r,n}(x)+f_{r,n}}\exp\left(-\frac{1}{2}\frac{z^2}{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)n}\right)\mathrm{d}z \nonumber\\ &\leq  \frac{2 f_{r,n}}{\sqrt{\mathcal{I}_{\sigma^2} (\sfrac{r}{n},\lambda^1)n}}\exp\left(-\frac{1}{2}\frac{(M_n^{*}(t^1)-s_{r,n}(M_n^{*}(t^1))-f_{r,n})^2}{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)n}\right). \label{equation:1st_bound_max_P}
		\end{align} 
		Regarding the definition of $f_{r,n}$, we split our considerations into two steps. First, we consider the case where $0< r\leq t_1$. We may assume that $\sigma_1>0$, as else we could consider the case $0<r\leq t_i$ for the minimal $i$ such that $\sigma_i>0$. In this case and for $v\in V_N^{'}$, we have  $\mathrm{Var}[S_v^N(t^1)-S_v^N(r)]= \mathcal{I}_{\sigma^2} (\sfrac{r}{n},\lambda^1)n$ and $f_{r,n}=C_f(\sigma_1^2r)^{\sfrac{2}{3}}.$
		To estimate the exponential on the right hand side of \eqref{equation:1st_bound_max_P}, we note that
		\begin{align}\label{equation:4.66}
			(M_n^{*}(t^1)-s_{r,n}(M_n^{*}(t^1))-f_{r,n})^2&\geq  M_n^{*}(t^1)^2\left(1-\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n})}{\mathcal{I}_{\sigma^2}(\lambda^1)}\right)^2 - 2f_{r,n} M_n^{*}(t^1)\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)}.
		\end{align}
		Inserting this into \eqref{equation:1st_bound_max_P} and computing the square, we obtain that \eqref{equation:1st_bound_max_P} is bounded from above by
		\begin{align}
			 &\frac{2 f_{r,n}}{\sqrt{\mathcal{I}_{\sigma^2} (\sfrac{r}{n},\lambda^1)t^1}}\exp\left(-\frac{1}{2}\frac{M_n^{*}(t^1)^2\left(1-\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n})}{\mathcal{I}_{\sigma^2}(\lambda^1)}\right)^2 - 2f_{r,n} M_n^{*}(t^1) \frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)}}{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)t^1}\right) \nonumber
			\\ &\quad\leq \frac{2 f_{r,n}}{\sqrt{\mathcal{I}_{\sigma^2} (\sfrac{r}{n},\lambda^1)t^1}} \exp\left(-2\log(2)t^1 \frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)} + \frac{1}{2}\log(t^1)\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)} \right. \nonumber
			\\ &\qquad \qquad \qquad \qquad \qquad \quad \left.-\frac{\log(t^1)^2}{32 \log(2)t^1}\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)}+\frac{C_f \sigma_1^{\sfrac{4}{3}}r^{\sfrac{2}{3}}}{(4\log(2))^{-\sfrac{1}{2}}\bar{\sigma}_1}\right) .\label{equation:2nd_bound_max_P}
		\end{align}
	Note, since $r\leq t_1$, $\frac{\frac{1}{\lambda_1}\mathcal{I}_{\sigma^2}(\lambda_1)}{\frac{1}{\lambda^1}\mathcal{I}_{\sigma^2}(\lambda^1)}=\frac{\sigma_1^2}{\bar{\sigma}_1^2}\in (0,1)$ and so we have
		\begin{align}
			\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)}t^1= t^1-t^1 \frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n})}{\mathcal{I}_{\sigma^2}(\lambda^1)}= t^1-r\frac{\frac{1}{\sfrac{r}{n}}\mathcal{I}_{\sigma^2}(\sfrac{r}{n})}{\frac{1}{\lambda^1}\mathcal{I}_{\sigma^2}(\lambda^1)}=t^1-r\frac{\frac{1}{\lambda_1}\mathcal{I}_{\sigma^2}(\lambda_1)}{\frac{1}{\lambda^1}\mathcal{I}_{\sigma^2}(\lambda^1)}=t^1-\eta_1 r,
		\end{align}
		for a $\eta_1<1$, independent of $r$ and $n$. Inserting this into \eqref{equation:2nd_bound_max_P}, we get
		\begin{align}\label{equation:3rdboundmaxP}
			A_{r,n,x}&\leq C r^{\sfrac{2}{3}} \exp\left(\tilde{C}r^{\sfrac{2}{3}}\right) 2^{-2(t^1-\eta_1 r)} \frac{\exp\left(\log(t^1)\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{2\mathcal{I}_{\sigma^2}(\lambda^1)}\right)}{\sqrt{\mathcal{I}_{\sigma^2} (\sfrac{r}{n},\lambda^1)t^1}} \exp\left(-\log(t^1)\frac{\log(t^1)}{32 \log(2)t^1}\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)}\right)\nonumber\\ &\leq  C 2^{-\eta_2 (t^1-r)+o(t^1-r)}.
		\end{align} 	
		As $\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)}<1,$ the fraction involving the square root in \eqref{equation:3rdboundmaxP} can be estimated as
		\begin{align}
			\frac{\exp\left[\log(t^1)\frac{1}{2}\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(1)}\right]}{\sqrt{\mathcal{I}_{\sigma^2} (\sfrac{r}{n},\lambda^1)t^1}}< \frac{1}{\sqrt{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}}, \label{equation:3rd_bound_max_P}
		\end{align}
		Using this in \eqref{equation:3rdboundmaxP}, we obtain in the case of $0<r\leq t_1$,
		\begin{align}
			A_{r,n,x}\leq C r^{\sfrac{2}{3}} \exp\left(\tilde{C}r^{\sfrac{2}{3}}\right)2^{-2(t^1-\eta_1 r)}\leq C 2^{-2(t^1-\eta_1 r)+o(r)}. \label{equation:5th_bound_max_P}
		\end{align}
		The same computation as in \eqref{equation:1st_bound_max_P}, now in the case of $t_1<r \leq t^1$,  $f_{r,n}=C_f(\mathcal{I}_{\sigma^2}(\frac{r}{n},\lambda^1)n)^{\sfrac{2}{3}}$ and $x \in I_n(1)$, yields
		\begin{align}
			A_{r,n,x} &\leq  \frac{2 f_{r,n}}{\sqrt{\mathcal{I}_{\sigma^2} (\sfrac{r}{n},\lambda^1)n}}\exp\left(-\frac{1}{2}\frac{(M_n^{*}(t^1)-s_{r,n}(M_n^{*}(t^1))-f_{r,n})^2}{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)t^1}\right)\nonumber\\ &\leq C 2^{-2t^1\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)}} (\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)n)^{\sfrac{1}{6}}\exp\left(\frac{1}{2}\log(t^1)\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)}+\frac{C_f(\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)n)^{\sfrac{2}{3}}}{(4\log(2))^{-\sfrac{1}{2}}\bar{\sigma}_1}\right). \label{equation:4.82}
		\end{align}
		Next, we observe that the second exponential is bounded by $(\mathcal{I}_{\sigma^2}(\frac{r}{n},\lambda^1)n)^{\sfrac{1}{2}}$, as seen in \eqref{equation:3rd_bound_max_P} and the fact that for $t_1<r <t^1$,
		\begin{align}
			t^1\frac{\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\mathcal{I}_{\sigma^2}(\lambda^1)}= \frac{  \frac{1}{\lambda^1-\sfrac{r}{n}}\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)}{\frac{1}{\lambda^1}\mathcal{I}_{\sigma^2}(\lambda^1)}(t^1-r)\geq \eta_2(t^1-r),
		\end{align}
		for a constant $\eta_2>1$ that is independent of $r$ and $n$. Using these in \eqref{equation:4.82}, we get
		\begin{align}
			A_{r,n,x}\leq C 2^{-2\eta_2(t^1-r)}(\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)n)^{\sfrac{2}{3}} \exp(\tilde{C}(\mathcal{I}_{\sigma^2}(\sfrac{r}{n},\lambda^1)n)^{\sfrac{2}{3}})\leq C 2^{-2 \eta_2 (t^1-r)+o(t^1-r)}. \label{equation:4th_bound_max_P}
		\end{align} 
		Combining the bounds in \eqref{equation:5th_bound_max_P} and \eqref{equation:4th_bound_max_P} and observing that both $(1-\eta_1)>0$ and $(1-\eta_2)<0$ hold, allows us to bound the sum in \eqref{equation:max_P_1} by an absolute constant $C_2>0$, i.e.
		\begin{align}
			\sum_{r=1}^{n-1} 2^{2(t^1-r)} \max_{x \in I_n(1)}A_{r,n,x} \leq  C\left[\sum_{r=1}^{t_1}2^{-2r(1-\eta_1)+o(r)}+\sum_{r=t_1 + 1}^{t^1-1}2^{2(1-\eta_2)(t^1-r)+o(t^1-r)}\right] \leq C_2.
		\end{align}
		Inserting this into \eqref{equation:1pcase_2nd_moment_1} finishes the proof in the one parameter case.
		We can bound $\mathbb{E}\left[h_N^2\right]$ from above as in the one parameter case (see \eqref{equation:1pcase_2nd_moment_1}),
		\begin{align}
		\mathbbm{E}[h_N^2] \leq \mathbbm{E}\left[h_N\right]^2+\mathbbm{E}\left[h_N\right]+\sum_{k=1}^{n-1} \sum_{\substack{v,w \in V_N^{'}\\r(v,w)=k}} \mathbbm{P} \left(C_{v;0,m}^N(t^m) \cap C_{w;0,m}^N(t^m) \right). \label{equation:mparam_2nd_moment_1}
		\end{align}
		We bound the last sum by bounding each summand. Let $v,w \in V_N^{'}$ with $r=r(v,w)\in\{1,\dotsc,n-1\}$ and $\tilde{k}(r) \in \{0,\dotsc,n-1\}$ such that $t^{\tilde{k}-1}\leq r <t^{\tilde{k}}$. We set $B_{k,n}(x)\coloneqq x-s_{k,n}(x)+[-f_{r,n},f_{r,n}]$. Then by dropping the condition for $w$ up to time $r$,
		\begin{align}
		\mathbbm{P} \left(C_{v;0,m}^N(t^m) \cap C_{w;0,m}^N(t^m)\right)&\leq \mathbbm{P}\left(C_{v;0,m}^N(t^m)\right) \max_{x \in I_n(\tilde{k})} \mathbbm{P}\left(S_w^N(t^{\tilde{k}})-S_w^N(r)\in B_{r,n}(x)\right) \nonumber \\
		&\quad\times \prod_{k= \tilde{k}}^{m-1} \max_{x \in I_n(k)} \mathbbm{P}\left({S_w^N(t^{k+1})-S_w^N( t^{k})\in B_{k,n}(x)}\right).
		\end{align}
		Note, $\mathbbm{P}\left(S_w^N(t^{\tilde{k}})-S_w^N(r)\in B_{r,n}(x)\right)$ and $\mathbbm{P}\left({S_w^N(t^{k+1})-S_w^N( t^{k})\in B_{k,n}(x)}\right)$ are terms that we have already considered in the one parameter case, and that each event considered here is also involving exactly one effective parameter.
		Thus for each effective parameter, we have analogue estimates as in \eqref{equation:3rdboundmaxP} and \eqref{equation:4th_bound_max_P}, now with constants $\eta_{1,k}, \eta_{2,k}$ as before, only that each now depends on the corresponding effective parameter.
		Further, for fixed $v \in V_N^{'}$, the number of points $w\in V_N^{'}$ with $d_N^{\infty}(v,w)\in [2^k,2^{k+1}],$ or equivalently $r(v,w) \in [n-k-1,n-k]$, is bounded by $c_1 2^{2k}$ for some $c_1>0$. Hence, we can bound the double sum on the right-hand side of \eqref{equation:mparam_2nd_moment_1} from above by
		\begin{align}
		c_1 \mathbbm{E}\left[h_N\right] &\sum_{r=1}^{t^m-1} 2^{2(t^m-r)} \max_{\substack{x \in I_n(\tilde{k})\\ v \in V_N^{'}}} \mathbbm{P}\left(S_w^N(t^{\tilde{k}})-S_w^N(r)\in  B_{r,n}(x)\right) \prod_{k= \tilde{k}+1}^{m}  \max_{x \in I_n(k)}\mathbbm{P}\left(S_w^N(t^k)-S_w^N( t^{k-1})\in B_{k-1,n}(x)\right)\nonumber\\
		&\leq C\mathbbm{E}[h_N]\sum_{r=1}^{t^m-1}2^{2(t^m-r)} (2^{-2(t^{\tilde{k}}-\eta_{1,\tilde{k}}r)} +2^{-2\eta_{2,\tilde{k}}(t^{\tilde{k}}-r)})\prod_{k=\tilde{k}+1}^{m} 2^{-2(t^{k} -\eta_{1,k} t^{k-1})} \nonumber \\
		&=C\mathbbm{E}[h_N]\sum_{r=1}^{t^m-1} [2^{2r(\eta_{1,\tilde{k}}-1)}+2^{2(1-\eta_{2,\tilde{k}})(t^{\tilde{k}}-r)}]\prod_{k=\tilde{k}+1}^{m-1} 2^{2t^k(\eta_{1,k+1}-1)}   \leq C_2 \mathbbm{E}[h_N].
		\end{align}
		In the last line we used that the last sum can be uniformly bounded by a constant and the last product is bounded from above by $1$.
		Inserting this into \eqref{equation:mparam_2nd_moment_1} allows to bound the second moment by $\mathbbm{E}[h_N]^2+ (1+C_2)\mathbbm{E}[h_N]$, which concludes the proof of \autoref{lemma:upboundon2ndmoment}.
	\end{proof}
\begin{proof}[Proof of \autoref{proposition:prop_lb_mibrw}] \label{proof:prop_lb_mibrw}
	Using the Paley-Zygmund inequality with \autoref{lemma:lboundon1stmoment} and \autoref{lemma:upboundon2ndmoment}, we obtain
	\begin{align}
	\mathbbm{P}(h_N \geq 1) &\geq \frac{\mathbbm{E}\left[h_N\right]^2}{\mathbbm{E}\left[h_N^2\right]}\geq \frac{\mathbbm{E}\left[h_N\right]^2}{\mathbbm{E}\left[h_N\right]^2+(1+C_2)\mathbbm{E}\left[h_N\right]}\geq  \frac{1}{1 + \frac{1+C_2}{\mathbbm{E}\left[h_N\right]}}\geq \delta_0,
	\end{align}
	for some constant $\delta_0 \in (0,1)$, uniformly in $N$.
\end{proof}

==> mbrw.tex <==
Let $N=2^n$ for some $n \in \mathbbm{N}$. For $v \in V_N$, let $\mathcal{B}_k^N (v)$ be the collection of subsets of $\mathbbm{Z}^2$ consisting of squares of size $2^k$ with lower left corner in $V_N$. Let $\{b_{k,B} \}_{k \geq 0 , B \in \mathcal{B}_k^N}$ denote an i.i.d. family of centred  Gaussian random variables with unit variance and set
\begin{equation}
	b_{k,B}^N \coloneqq \begin{cases}
							b_{k,B}, \, B \in \mathcal{B}_k^N, \\
							b_{k,B^{'}}, \, B \sim_N B^{'} \in \mathcal{B}_k^N.
						\end{cases}
\end{equation}
\begin{definition}[Modified inhomogeneous branching random walk (MIBRW)]
	The modified inhomogeneous branching random walk (MIBRW) $\{S_v^N\}_{v \in V_N}$ is defined by
	\begin{equation}\label{equation:def_MIBRW}
		S_z^N (t) \coloneqq \sum_{k=n-t}^{n} \sum_{B \in \mathcal{B}_k^N (z)} 2^{-k} \sigma\left(\frac{n-k}{n}\right) b_{k,B}^N,
	\end{equation}
	where $0 \leq t \leq n,$ $t \in \mathbbm{N}$ and $\sigma$ is defined as in \eqref{parameters1}.
\end{definition}
Note that $\{S_v^N\}_{v\in V_N}$ is a Gaussian field but not a time-inhomogeneous branching random walk. The key point is that it interpolates between the time-inhomogeneous branching random walk $\mathcal{R}_{v}^{N}$ and the scale-inhomogeneous DGFF $\psi^N_v$. In order to do so, we aim to approximate its correlations which mainly depend on the distance between the corresponding two points on the grid. If we now fix a single grid as in the case of the time-inhomogeneous branching random walk, we obviously do make severe mistakes by separating nearby points that lie in neighbouring boxes, which makes them independent in the approximation already on large scales and thus leading to small correlations. In the definition of the modified branching random walk one tries to circumvent this problem by taking the uniform average over all possible grids with the restriction of boxes having to have their lower left corner in $V_N$. In the inner quarter of the field this turns out to be a better approximation of the Euclidean distance which governs the correlation structure. The justification for this idea comes with \autoref{lemma:cov_comp}.


==> outline_proof.tex <==



==> scale_dep_brw.tex <==
In this section, we present the time-inhomogeneous branching random walk with finitely many macroscopic changes in the variance, introduced by Ouimet in \cite{2015arXiv150908172O}. This generalizes the model considered by Fang and Zeitouni in \cite{MR2968674}, where they consider the case in which the variance changes exactly once at half the time.
Our particular interest in this model is due to the fact that the scale-inhomogeneous Gaussian free field is the perfect analogue in the context of Gaussian free fields.\\
We begin with constructing a $4$-ary tree structure, $4$-ary so that we can easily compare results to the scale-inhomogeneous Gaussian free field, introduced in \autoref{sec:scale_GFF}. The depth of the tree is indexed by time $t\in \mathbbm{N}$.  At time $t=0$, there exists exactly one particle $o$, called the origin, and we set $\mathbbm{D}_0=\{o\}$, the set of particles at time $t=0$. At time $t=1$, four new particles are born and linked to $o$ both by an edge. $\mathbbm{D}_1$ is the set of particles at time $t=1$. At time $t=k$, we iterate this step for each particle present at time $k$. So, at time $t=n$, we end up with a set of particles $\mathbbm{D}_n$, consisting of $N^2=2^{2n}$ elements.
For $v\in \mathbbm{D}_n$, we denote by $v_k$ the ancestor of $v$ at time $k$, which is the unique particle $w \in \mathbbm{D}_k$ that intersects the shortest path from the origin $o$ to $v$.
There is also a natural distance induced by the tree, i.e. for $u,v \in \mathbbm{D}_n$, we denote by
$\rho(u,v)= \max\{k\in \{0,\dotsc,n\}:\,u_k=v_k\}$, the latest time at which $u$ and $v$ shared a common ancestor. Next, we introduce the scale- and variance parameters. Fix $M\in \mathbbm{N}$, the number of scales, and let
\begin{align}
	&\sigma=(\sigma_1,\dotsc,\sigma_M) \in (0,\infty)^M \qquad & \text{(variance parameters)},\\
	&\lambda=(\lambda_1,\dotsc,\lambda_M) \in (0,1]^M \qquad &\text{(scale parameters)},
\end{align}
where $0\eqqcolon \lambda_0 <\lambda_1<\dotsc <\lambda_M \coloneqq 1$. We can encode them both into the left-continuous step function $\sigma(s)\coloneqq \sigma_1 \mathbbm{1}_{0}(s)+ \sum_{i=1}^{M} \sigma_i \mathbbm{1}_{(\lambda_{i-1},\lambda_i]}(s),$ for $s\in [0,1]$. For simplicity, we assume that $\lambda_i n \in \mathbbm{N}$, for any $i,n\in \mathbbm{N}$.
\begin{definition}\label{def:BRW}
	The $(\sigma,\lambda)-$BRW (branching random walk) in time $n$ is a collection of positively correlated random walks $\{\{S_v(t)\}_{t=0}^{n}\}_{v \in \mathbbm{D}_n}$, defined by
	\begin{align}
		S_v(t) \coloneqq \sum_{i=1}^{M}\sum_{k=\lambda_{i-1}n+1}^{\lambda_i n \wedge t}\sigma_i Z_{v_k},\qquad t\in \{0,\dotsc,n\}, &v\in \mathbbm{D}_n,
	\end{align}
	where $\{Z_{v_k}\}_{k\in \{0,\dotsc,n\};v\in \mathbbm{D}_n}$ is a family of i.i.d $\mathcal{N}(0,1)$ random variables.
\end{definition}
As already noted by Bovier and Kurkova in \cite{MR2070334} and \cite{MR2070335}, in the context of GREM (generalized random energy model, a certain type of Gaussian process indexed by trees) and later in \cite{MR3351476} by Bovier and Hartung in the case of the time-inhomogeneous BBM (branching Brownian motion), the continuous analogue of time-inhomogeneous BRW, the concave hull of $\mathcal{I}_{\sigma^2}(t)=\int_{0}^{t}\sigma^2(s)\mathrm{d}s$, denoted by $\hat{\mathcal{I}}_{\sigma^2}$, plays a crucial role for the investigation of the extremes. As $\sigma(s)$ is left-continuous, piecewise constant with a finite number of jumps, it is easy to see that it exists a unique function $\bar{\sigma}(s),\,s\in [0,1]$, such that for any $s\in [0,1]$, it holds $\hat{\mathcal{I}}_{\sigma^2}(s)= \mathcal{I}_{\bar{\sigma}^2}(s)$ . Clearly, $\bar{\sigma}(s)$ is positive, piecewise constant, non-increasing with finitely many jumps, i.e. it takes the form $\bar{\sigma}(s)=\bar{\sigma}_1 \mathbbm{1}_0(s)+ \sum_{i=1}^{m} \bar{\sigma}_i \mathbbm{1}_{(\lambda^{i-1},\lambda^i]}(s)$, where $m\leq M$ and $0=\lambda^0<\dotsc<\lambda^m=1$, with $\{\lambda^0,\dotsc,\lambda^m\}\subset \{\lambda_0,\dotsc,\lambda_M\}$.
Ouimet in \cite{2015arXiv150908172O} proved the following:
\begin{thm}\label{thm:2nd_order_ibrw}
	Let $n \in \mathbbm{N}$, $N=2^n$ and  $\{\{S_v(t)\}_{t=0}^{n}\}_{v \in \mathbbm{D}_n}$ a $(\sigma,\lambda)-$BRW. Assume that on each interval $[\lambda^{i-1},\lambda^i]$, for $i=1,\dotsc,m$, we have either $\mathcal{I}_{\sigma^2}\equiv \mathcal{I}_{\bar{\sigma}^2}$ or $\mathcal{I}_{\sigma^2}< \mathcal{I}_{\bar{\sigma}^2}$. Then, in probability:
	\begin{align}
		&\lim\limits_{N \rightarrow \infty} \frac{\max_{v \in \mathbbm{D}_n}S_v(n)-\frac{\gamma^*}{\sqrt{\log(2)}\log(N^2)}-\sum_{i=1}^{m}\frac{\omega_i}{2}\frac{\bar{\sigma}_i}{2\sqrt{\log(2)}}\log((\lambda^i-\lambda^{i-1})n)}{\log(\log(N))}=0,
	\end{align}
	where $\gamma^*=\mathcal{I}_{\bar{\sigma}}(1)=\sum_{i=1}^{m}\bar{\sigma}_i (\lambda^{i}-\lambda^{i-1})$ and
	\begin{equation}
		w_j= \begin{cases}
		3, \quad \hat{I}_{\sigma^2}|_{( \lambda^{j-1},\lambda^j]} \equiv I_{\sigma^2}|_{(\lambda^{j-1},\lambda^j]} \\
		1, \quad else.
		\end{cases}
	\end{equation}
\end{thm}
This answers the question about the second order behaviour of the maximum, when there are finitely many macroscopic changes of variance, raised by Fang and Zeitouni in \cite{MR2968674}, where the authors treated the case of exactly one change of variance at half the time. Of general importance, they have already noticed that in the case of strictly increasing variance parameter $\sigma$, the time-inhomogeneous BRW in time $n$ behaves like $2^{2n}$ i.i.d. centred Gaussian random variables with the identical variance, $\mathcal{I}_{\sigma^2}(1)n$. To get the full picture, Ouimet essentially adapted their proof to the more general case, i.e. it relies on modified first and second moment methods in combination with large deviation heuristics, to identify "optimal paths", which serve as localizers for the second moment analysis to avoid blow-up of the second moment, and Brownian bridge estimates.
An interesting fact, that follows from the proof, is that particles to be maximal at the end, have a high probability to be close to the maximum at the times $t^i$, for $i=1,\dotsc,m$. The adaptation to more general tree structures, in particular supercritical Galton-Watson trees, is immediate. Similar results in the case of more general increments and trees have been proved by Mallein in \cite{MR3361256} and \cite{MR3373310}. 

==> sketch_proof.tex <==
The idea for the proof of \autoref{theorem:thm_second_order_correction} is as in the case of the 2d DGFF \cite{MR2846636}, i.e. one constructs auxiliary Gaussian fields, a time-inhomogeneous BRW and an inhomogeneous modified branching random walks (IMBRW) that approximately share the correlation structure with the scale-inhomogeneous DGFF and additionally have an (approximate) hierarchical structure. Using Gaussian comparison, namely \autoref{thm:sudakov}, we can bound the expected maximum of the scale-inhomogeneous DGFF from above by the expected maximum of the time-inhomogeneous BRW which is explicitly known \cite[Theorem~1.4]{MR3361256}\cite{2015arXiv150908172O}. In a second step we use Gaussian comparison to show that the expected maximum of the scale-inhomogeneous DGFF can be bounded from below by the expected maximum of the IMBRW when neglecting contributions from large scales. In order to control their influence on the maximum value, one uses a Gaussian perturbation argument. For the remaining inner part, we  need to determine the expected maximum of the IMBRW. The advantage in this case is that the IMBRW exhibits an approximate hierarchical structure that allows us to perform a multi-scale second moment method in which we combine ideas from the 2d DGFF and time-inhomogeneous BRW/BBM.
The principle idea to prove \autoref{theorem:thm_tightness} is to compare the distribution of the centred maximum of the scale-inhomogeneous DGFF with the distribution of the centred IMBRW and then prove tail estimates for the centred maximum of the IMBRW that allow us to deduce tightness. This is again based on Gaussian comparison, just that this time we use \autoref{thm:slepian} in the place of \autoref{thm:sudakov}, which allows to control distributions instead of expectations. Tail estimates for the auxiliary process are then provided using a modified multi-scale second moment analysis. In our proof we use ideas from \cite{MR3433630} \cite{2015arXiv150304588D}\cite{MR3262484}.


==> summary.tex <==
This thesis studies the behaviour of the maximum of the two-dimensional scale-inhomogeneous discrete Gaussian Free Field, introduced by Ouimet and Louis-Pierre in \cite{MR3541850}, which in turn generalizes the model considered in !!!pierre zindy!!!. In short,
In \cite{MR3541850}, Ouimet and Lious Pierre determined the first order convergence of the maximum, as well as the number of $\gamma-$high points.
We generalize the first order convergence, by proving first a second order correction on the expected maximum and second additional tail estimates on the centred maximum, which imply tightness of the centred maximum.

==> summary_openquestions.tex <==
As we have identified the second order correction and proved tightness of the centred maximum $\left\{\psi^N_v-\mathbbm{E}\left[\psi_N^{*} \right]\right\}_{N\in \mathbbm{N}}$, we have convergence in distribution of a subsequence. Naturally, we would like to extend this to the entire sequence and, of course, identify the limit. This will be dealt with in the case of strictly increasing variance parameters in the second paper in this series.
Moreover, analogously to the case of the homogeneous discrete Gaussian free field and the case of inhomogeneous branching Brownian motion, we expect convergence of the extremal process $\eta_N= \sum_{v\in V_N} \mathbbm{1}_{v\,\text{loc. max.}}\delta_{v/N}\otimes \delta_{\psi_v^N-\psi_N^{*}}$ and the formation of so called clusters processes of extremal particles, that should form due to the correlation structure. Particles near local extrema are as the entire field heavily correlated and thus, expected to be unusually large as well, which form the so-called clusters. Moreover, it is known in the case of DGFF that these clusters share the same law, and are independent of each other. In our case, we expect similar things to happen, that should now depend on the parameters of the field. In particular, in the weakly correlated regime of strictly increasing variance, this should be actually easier than in the case of the usual DGFF. A first step in this direction would be to understand the distribution of local extrema in the field, which will be done in the case of strictly increasing variance in a third paper.


==> tgff.tex <==
One key difference between the two-dimensional GFF with Dirichelet boundary condition and the one dimensional BRW lies in the additional difficulty that due to the zero boundary conditions, the covariance estimates near the boundary break down and that the variance, in general, is not the same at all points of $V_N$. The Torus GFF (TGFF) $\{\tilde{Y}_v^N\}_{v \in V_N}$ is a Gaussian field whose correlation structure resembles that of the GFF with the important advantage, that its variance is constant across $V_N$. To define it formally, we need some additional notation. For $x,y \in \mathbbm{Z}^2$ write $x \sim_N y$ if $x-y \in (N\mathbbm{Z})^2$. Similarly, for $B,B^{'} \subset V_N$, write $B \sim_N B^{'}$ if there exist integers $i,j \in \mathbbm{Z}$ such that $B^{'} = B + (iN,jN).$ Let $\tau$ denote an exponential random variable with parameter $\frac{1}{N^2}$ and let $\{W_m\}_{m \in \mathbbm{N}}$ be a simple random walk on the torus independent of $\tau$. For $x,y \in V_N$ let
\begin{equation}\label{tgff_kernel}
	\bar{G}_N (x,y) \coloneqq \frac{\pi}{2} \mathbbm{E}_{x}\left[\sum_{m=0}^{\tau}\mathbbm{1}_{W_m \sim_N y}\right],
\end{equation}
where $\mathbbm{E}_x$ denotes expectation over both $\tau$ and the random walk $W_m$ started at $x$. In other words, $\bar{G}_N (x,y)$ is the renormalised Green function of a simple random walk on the torus of side $N$ killed at the independent exponential time $\tau$.
\begin{definition} [Torus GFF]
	The torus GFF (TGFF) on $V_N$ is a centred Gaussian process $\{\tilde{Y}_v^N\}_{v \in V_N}$ with covariance given by the Green function $\bar{G}_N$ as in \eqref{tgff_kernel}.
\end{definition}
Note that we need to define a stopping time $\tau$ that is of the same order as the hitting time of the boundary in the GFF, since on the torus we are border-less. The absence of a border and the fact that the simple random walk is symmetric gives that for $x,y \in V_N$ we have $\mathbbm{E}\left[(\tilde{Y}_x^N)^2\right]= \mathbbm{E}\left[(\tilde{Y}_y^N)^2\right].$ Moreover, we have the estimate (see \cite[Theorem 1.6.2]{MR2985195})  
\begin{equation}\label{tgff_var}
	\left| \mathbbm{E}\left[(\tilde{Y}_x^N)^2\right]- \log(N)\right| \leq C,
\end{equation}
where the constant $C$ does not depend on $N$.
To be able to compare with our scale-inhomogeneous GFF $\{\psi_n^N\}_{v\in V_N}$, we have to modify the variance along scales in the same way.
\begin{definition}[Scale-Inhomogeneous TGFF]
	Let $\{\tilde{Y}_v^N\}_{v \in V_N}$ be a TGFF on $V_N$. With previous notations, we define the scale-inhomogeneous torus Gaussian Free Field $\{Y_v^N\}_{v \in V_N}$:
	\begin{equation}
		Y_v^N\coloneqq \sum_{i=1}^{M} \sigma_i \nabla \tilde{Y}_v^N (\lambda_i).
	\end{equation}
\end{definition}
Regarding Equation \eqref{tgff_var} combined with the definition and independence of increments, which are piecewise homogeneous, then gives
\begin{equation}\label{si_tgff_var}
\left| \mathbbm{E}\left[(Y_x^N)^2\right]- \log(N)\sum_{i=1}^{M} \sigma_i^2\right| \leq C.
\end{equation}


==> tightness.tex <==
In this section, we will use our previous result on the second order correction for the scale-inhomogeneous GFF $\psi_N$ to derive tightness. Therefore, we use an argument used before for branching random walks, namely the Dekking-Host argument (cf. \cite[Lemma 9]{zeitouni2012branching}):

\begin{lemma}[Dekking-Host] \label{lemma:dekking_host}
	Let $\psi^N, \tilde{\psi}^N$ be two independent $(\sigma, \lambda)$- GFF on $V_N$. Then,
	\begin{equation}
		\mathrm{E}[|\psi_N^* - \tilde{\psi}_N^* |] \leq 2 \mathrm{E}[\psi_{4N}^*- \psi_N^*].
	\end{equation}
	\begin{proof}
		We decompose $V_{4N}$ into sixteen disjoint boxes of side $N$, where we assume wlog $N=2^n$ for some $n\in \mathbbm{N}$, as usually. Then, by definition and \autoref{lemma:cov_comp} we have $\mathrm{E}[(\psi_v^{4N}-\psi_w^{4N})^2]\geq \mathrm{E}[(\psi_v^{N,i}-\psi_w^{N,i})^2],$ for $i=1,2$ and $v,w\in (iN,iN)+V_N$, where $\{\psi_v^{N,i}\}_{v \in  (iN,iN)+V_N}$ are two independent $(\sigma, \lambda)$-GFF on $V_N$. Applying \autoref{thm:sudakov}, we obtain:
		\begin{equation}
			\mathrm{E}[\psi_{4N}^*]\geq \mathrm{E}[\max_{i=1}^2 \psi_N^{*,i}].
		\end{equation}
		With the observation that $\max(a,b)= \frac{a+b+|a-b|}{2}$, we finally get
		\begin{equation}
			\mathrm{E}[\psi_{4N}^*]\geq \mathrm{E}[\max_{i=1}^2 \psi_N^{*,i}] \geq \mathrm{E}[\psi_N^*] + \frac{\mathrm{E}[| \psi_N^{*,1}-\psi_N^{*,2}|]}{2}.
		\end{equation}
		This proves the claim.
	\end{proof}
\end{lemma}
\begin{rem}
	Note that this Lemma reduces the issue of tightness of $\{\psi_N^* - \mathrm{E}[\psi_N^*] \}_{N\geq 0}$ to a control on a lower bound on $\mathrm{E}[\psi_{2N}]$, which should differ from an upper bound on $\mathrm{E}[\psi_N^*]$ only by a constant. This is made precise in the following Lemma.
\end{rem}
\begin{lemma}\label{lemma:tightness}
	Let $\{A_n\}_{n \in \mathbbm{N}}$ be a sequence of real valued random variables and $\{\tilde{A}_n\}_{n \in \mathbbm{N}}$ an independent copy, such that for all $n \in \mathbbm{N}$
	\begin{equation}
		\mathrm{E}[|A_n - \tilde{A}_n |] \leq C,
	\end{equation}
	where $C>0$ is a constant independent of $n$.\\ Then, $\mathrm{E}[A_n]$ exists and $\{A_n - \mathrm{E}[A_n] \}_{n \in \mathbbm{N}}$ is tight, i.e.
	\begin{equation}
		\mathbbm{P}[|A_n - \mathrm{E}[A_n]| \geq K] \leq f(K),
	\end{equation}
	for some function $f$, such that $f(K) \rightarrow 0$ as $K \rightarrow \infty$.
	\begin{proof}
		Fix $n \in \mathbbm{N}$ and let $A_n, \tilde{A}_n$ as above, then
		\begin{align}
			C \geq \mathrm{E}[|A_n - \tilde{A}_n|] = \mathrm{E}[|A_n - \tilde{A}_n| | A_n] \overset{\text{Jensen}}{\geq} \mathrm{E}[|\mathrm{E}[A_n - \tilde{A}_n | A_n]|] \\ \overset{\tilde{A}_n \text{ independent of } A_n}{=} \mathrm{E}[| \tilde{A}_n - \mathrm{E}[A_n]|] \overset{\tilde{A}_n \sim A_n}{=} \mathrm{E}[| A_n - \mathrm{E}[A_n]|].
		\end{align}
		With the Markov inequality it follows:
		\begin{equation}
			\mathbbm{P}(|A_n - \mathrm{E}[A_n]| > K)\leq \frac{\mathrm{E}[|A_n - \mathrm{E}[A_n]|]}{K} \overset{K \rightarrow \infty}{\rightarrow} 0.
		\end{equation}
		Since all computations hold uniformly in $n$, the statement follows.
	\end{proof}
\end{lemma}

Now, we have everything together to prove \autoref{theorem:thm_tightness}:
\begin{proof}[Proof of \autoref{theorem:thm_tightness}]
	By \autoref{theorem:thm_second_order_correction} we have $\mathrm{E}[\psi_N^*]= m_N + O(1).$ Moreover, 
	\begin{equation}
		| m_{4N} - m_N| \leq D,
	\end{equation}
	for a constant $D>0$ independent of $N$.
	Thus, by \autoref{lemma:dekking_host} we have
	\begin{equation}
		\mathrm{E}[|\psi_N^* - \tilde{\psi}_N^*| ] \leq C,
	\end{equation}
	for a constant $C>0$ uniformly in $N$. Then, by \autoref{lemma:tightness} the statement follows.
\end{proof}

==> upper_bound.tex <==
The goal in this section is to prove the upper bound in \autoref{theorem:thm_second_order_correction}. We first relate the maxima of the scale-inhomogeneous DGFF with those of the MIBRW.
\begin{lemma}\label{lemma:up_bound_lemma}
	Let $\{ g_v \}_{v \in V_N}$ denote a collection of independent identically distributed standard Gaussian random variables. Then, there is a finite constant $C_1$ such that 
		\begin{equation}
			\mathbbm{E}\left[\psi_N^*\right] \leq \sqrt{\log(2)} \mathbbm{E}\left[\max_{v \in V_N}\left( S_v^N + C_1 g_v\right)\right].
		\end{equation}
	\begin{proof}
	First, write $V_N^{'}= V_N+ (2N,2N) \subset V_{4N}$. By the Gibbs-Markov property for the underlying DGFF we can find a constant $\tilde{C}>0$, uniformly in $N$, such that for $v,w \in V^\prime_N$,
		\begin{equation}
			\mathbbm{E}\left[(\psi_v^N - \psi_w^N)^2\right]\leq \mathbbm{E}\left[(\psi_v^{4N}-\psi_w^{4N})^2\right]+ \tilde{C}.
		\end{equation}
	Further, for $v,w \in V_N$ we write $v_N = v + (2N,2N)$ and $w_N = w +(2N,2N)$. By \autoref{lemma:cov_comp} $iv.$,
		\begin{equation}
				\mathbbm{E}\left[(\psi_{v_N}^{4N}- \psi_{w_N}^{4N})^2\right] \leq \log(2) \mathbbm{E}\left[(S_v^N - S_w^N)^2\right]+\bar{C}.
		\end{equation}
	Thus, we can apply Sudakov-Fernique and get
		\begin{equation}
			\mathbbm{E}\left[\max_{v \in V_N} \psi_v^N\right]\leq    \log(2) \mathbbm{E}\left[\max_{v \in V_N}S_v^N+ C_1 g_v\right],
		\end{equation}
	where $\{g_{v}\}_{v \in V_N}$ form a family of independent standard Gaussian random variables and where $C_1>0$ is a constant independent of $N$.
	\end{proof}
\end{lemma}
\begin{prop}\label{proposition:1}
	There is a finite constant $C_2$, such that
	\begin{equation}
	\mathbbm{E}[\max_{v \in V_N}\psi_v^N] \leq \sqrt{ \log(2)} \mathbbm{E}\left[\max_{v \in V_N}R_v^N\right]+ C_2.
	\end{equation}
	\begin{proof}
		For $v,w \in V_N$, we have $\mathbbm{E}\left[(R_v^N)^2\right]= \mathbbm{E}\left[(S_v^N)^2\right]$ and $\mathbb{E}\left[R^N_v R^N_w\right]\leq \mathbb{E}\left[S^N_v S^N_w\right] + C.$ Together they imply
		\begin{align}
		\mathbbm{E}\left[(S_v^N- S_w^N)^2\right]\leq  \mathbbm{E}\left[(R_v^N- R_w^N)^2\right].
		\end{align}
		By Sudakov-Fernique in combination with \autoref{lemma:up_bound_lemma}, we find
		\begin{equation}
		\mathbbm{E}\left[\max_{v \in V_N}\psi^N_v\right]\leq \mathbbm{E}\left[\max_{v \in V_N}R_v^N+\bar{C}_1 g_v\right],
		\end{equation}
		with $\{g_v\}_{v \in V_N}$ being a family of independent standard Gaussian random variables.
		\end{proof}
\end{prop}
An application of \cite[Theorem 1.4]{MR3361256} yields that the time-inhomogeneous branching random walk $R^N$ satisfies
\begin{equation}\label{max_ibrw}
\mathbbm{E}\left[\max_{v \in V_N}R_v^N\right]=2 \sqrt{ \log(2)}\sum_{j=1}^{m} \bar{\sigma}_j \nabla \lambda^j n - \frac{(w_j \bar{\sigma}_j \log(\nabla \lambda^j n))}{4\sqrt{\log(2)}} + O(1).
\end{equation}
\autoref{proposition:1} yields the desired upper bound in \autoref{theorem:thm_second_order_correction}.
